Seeing Behind the Camera: Identifying the Authorship of a Photograph

We introduce the novel problem of identifying the photographer behind a photograph. To explore the feasibility of current computer vision techniques to address this problem, we created a new dataset of over 180,000 images taken by 41 well-known photographers. Using this dataset, we examined the effectiveness of a variety of features (low and high-level, including CNN features) at identifying the photographer. We also trained a new deep convolutional neural network for this task. Our results show that high-level features greatly outperform low-level features. We provide qualitative results using these learned models that give insight into our method's ability to distinguish between photographers, and allow us to draw interesting conclusions about what specific photographers shoot. We also demonstrate two applications of our method.

==> Makefile <==
## MAKEFILE FOR CVPR
## 11/3/2015

PDFLATEX	?= pdflatex -halt-on-error -file-line-error
BIBTEX		?= bibtex
MAKEGLOSSARIES ?= makeglossaries

ifneq ($(QUIET),)
PDFLATEX	+= -interaction=batchmode
ERRFILTER	:= > /dev/null || (egrep ':[[:digit:]]+:' *.log && false)
BIBTEX		+= -terse
else
PDFLATEX	+= -interaction=nonstopmode
ERRFILTER=
endif

## Action for 'make view'
OS=$(shell uname -s)
ifeq ($(OS),Darwin)
PDFVIEWER	?= open
else
PDFVIEWER	?= xdg-open
endif
TARGET = photographer
TARGETS += $(TARGET)
TEXTARGETS = $(TARGETS:=.tex)
PDFTARGETS = $(TARGETS:=.pdf)
AUXFILES   = $(TARGETS:=.aux)
LOGFILES   = $(TARGETS:=.log)
BIBFILES = $(patsubst %,%.bib,\
		$(shell grep '^[^%]*\\bibliography{' $(TEXTARGETS) | \
			grep -o '\\bibliography{[^}]\+}' | \
			sed -e 's/^[^%]*\\bibliography{\([^}]*\)}.*/\1/' \
			    -e 's/, */ /g'))
INCLUDEDTEX = $(patsubst %,%.tex,\
		$(shell grep '^[^%]*\\\(input\|include\){' $(TEXTARGETS) | \
			grep -o '\\\(input\|include\){[^}]\+}' | \
			sed -e 's/^.*{\([^}]*\)}.*/\1/' \
			    -e 's/\.tex$$//'))
AUXFILES += $(INCLUDEDTEX:.tex=.aux)

SPACE = $(empty) $(empty)
.PHONY: all clean pdf view snapshot distill distclean
all: pdf $(AFTERALL)
pdf: $(PDFTARGETS)
view: $(PDFTARGETS)
	$(PDFVIEWER) $(PDFTARGETS)

# define a \Revision{} command you can include in your document's preamble.
# especially useful with e.g. draftfooter.sty or fancyhdr.
# usage: \input{revision}
#        ... \Revision{}
ifneq ($(REVISION),)
REVDEPS += revision.tex
revision.tex: $(VCSTURD)
	/bin/echo '\newcommand{\Revision}'"{$(subst _,\_,$(REVISION))}" > $@
AUXFILES += revision.aux
endif

.INTERMEDIATE: $(AUXFILES)
%.aux: %.tex $(REVDEPS)
	$(PDFLATEX) -draftmode $* $(ERRFILTER)

ifneq ($(strip $(BIBFILES)),)
BIBDEPS = %.bbl
%.bbl: %.aux $(BIBFILES)
	$(BIBTEX) $*
endif

HAS_GLOSSARIES = $(shell \
		grep '^[^%]*\\printglossar\(ies\|y\)' $(TEXTARGETS) $(INCLUDEDTEX) && \
		echo HAS_GLOSSARIES)
ifneq ($(HAS_GLOSSARIES),)
GLSDEPS = %.gls
%.gls: %.aux
	$(MAKEGLOSSARIES) $(TARGETS)
endif

$(PDFTARGETS): %.pdf: %.tex %.aux $(GLSDEPS) $(BIBDEPS) $(INCLUDEDTEX) $(REVDEPS)
	$(PDFLATEX) $* $(ERRFILTER)
ifneq ($(strip $(BIBFILES)),)
	@if egrep -q "undefined (references|citations)" $*.log; then \
		$(BIBTEX) $* && $(PDFLATEX) $* $(ERRFILTER); fi
endif
	@while grep -q "Rerun to" $*.log; do \
		$(PDFLATEX) $* $(ERRFILTER); done

DRAFTS := $(PDFTARGETS:.pdf=-$(REVISION).pdf)
$(DRAFTS): %-$(REVISION).pdf: %.pdf
	cp $< $@
snapshot: $(DRAFTS)

%.distilled.pdf: %.pdf
	gs -q -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ \
		-dCompatibilityLevel=1.5 -dPDFSETTINGS=/prepress -c .setpdfwrite -f $<
	exiftool -overwrite_original -Title="" -Creator="" -CreatorTool="" $@

distill: $(PDFTARGETS:.pdf=.distilled.pdf)

distclean: clean
	$(RM) $(PDFTARGETS) $(PDFTARGETS:.pdf=.distilled.pdf) $(EXTRADISTCLEAN)

clean:
	$(RM) $(foreach T,$(TARGETS), \
		$(T).bbl $(T).bcf $(T).bit $(T).blg \
		$(T)-blx.bib $(T).brf $(T).glg $(T).glo \
		$(T).gls $(T).glsdefs $(T).glx \ $(T).gxg \
		$(T).gxs $(T).idx $(T).ilg $(T).ind \
		$(T).ist $(T).loa $(T).lof $(T).lol \
		$(T).lot $(T).maf $(T).mtc $(T).nav \
		$(T).out $(T).pag $(T).run.xml $(T).snm \
		$(T).svn $(T).tdo $(T).tns $(T).toc \
		$(T).vtc $(T).url $(T).synctex.gz $(T).dvi $(T).log $(T).pdf) \
		$(REVDEPS) $(AUXFILES) $(LOGFILES) \
		$(EXTRACLEAN)
	$(RM) *.log
